A Critical Reexamination of Intra-List Distance and Dispersion

Diversification of recommendation results is a promising approach for coping with the uncertainty associated with users' information needs. Of particular importance in diversified recommendation is to define and optimize an appropriate diversity objective. In this study, we revisit the most popular diversity objective called intra-list distance (ILD), defined as the average pairwise distance between selected items, and a similar but lesser known objective called dispersion, which is the minimum pairwise distance. Owing to their simplicity and flexibility, ILD and dispersion have been used in a plethora of diversified recommendation research. Nevertheless, we do not actually know what kind of items are preferred by them. We present a critical reexamination of ILD and dispersion from theoretical and experimental perspectives. Our theoretical results reveal that these objectives have potential drawbacks: ILD may select duplicate items that are very close to each other, whereas dispersion may overlook distant item pairs. As a competitor to ILD and dispersion, we design a diversity objective called Gaussian ILD, which can interpolate between ILD and dispersion by tuning the bandwidth parameter. We verify our theoretical results by experimental results using real-world data and confirm the extreme behavior of ILD and dispersion in practice.

==> arXiv/alg-greedy.tex <==
\begin{algorithm}[t] %[tbp]
\caption{Greedy heuristic.}
\label{alg:greedy}
\small
\begin{algorithmic}[1]
    \Require
    diversity objective $\divf: 2^{[n]} \to \bbR_+$;
    \# items $k \in [n]$.
    \State \textbf{for } $\ell = 1 \To k$ \textbf{do }
    $i_\ell \leftarrow \argmax_{i \in [n] \setminus \{ i_1, \ldots, i_{\ell-1} \}} \divf(\{i_1, \ldots, i_{\ell-1}, i\}) $.
    \State \textbf{return} $\{ i_1, \ldots, i_k \}$.
\end{algorithmic}
\end{algorithm}


==> arXiv/fig-GILD.tex <==
\begin{figure}[t]
    \centering%
    \null\hfill
    \subfloat[$k=16$.]{\includegraphics[width=.49\hsize]{fig/trade_ml_svd_16.pdf}}%
    \hfill
    \subfloat[$k=128$.]{\includegraphics[width=.49\hsize]{fig/trade_ml_svd_128.pdf}}%
    \hfill\null
    \caption{Trade-off between ILD and dispersion.
    For each value of $\sigma$, we plot $\ILD(S_{\GILD_\sigma,k}^\Gr)$ and $\disp(S_{\GILD_\sigma,k}^\Gr)$.
    }
    \label{fig:trade_ml_svd}
\end{figure}


==> arXiv/fig-plot_circles.tex <==
\begin{figure*}[t]
    \centering
    \null\hfill
    \subfloat[$128$ points chosen by ILD.\label{fig:plot_circles_ILD}]{\includegraphics[width=.25\textwidth]{fig/plot_art1_ILD-crop.pdf}}%
    \hfill
    \subfloat[$128$ points chosen by dispersion.\label{fig:plot_circles_disp}]{\includegraphics[width=.25\textwidth]{fig/plot_art1_disp-crop.pdf}}%
    \hfill
    \subfloat[$128$ points chosen by GILD.\label{fig:plot_circles_GILD}]{\includegraphics[width=.25\textwidth]{fig/plot_art1_GILD-crop.pdf}}%
    \hfill\null
    \caption{
    $128$ points (big red circles) of \circles selected by greedily maximizing each objective with the Euclidean distance.}
    \label{fig:plot_circles}
\end{figure*}


==> arXiv/fig-plot_ellipse.tex <==
\begin{figure*}[t]
    \centering
    \null\hfill
    \subfloat[$128$ points chosen by ILD.\label{fig:plot_ellipse_ILD}]{\includegraphics[width=.25\textwidth]{fig/plot_art2_ILD-crop.pdf}}%
    \hfill
    \subfloat[$128$ points chosen by dispersion.\label{fig:plot_ellipse_disp}]{\includegraphics[width=.25\textwidth]{fig/plot_art2_disp-crop.pdf}}%
    \hfill
    \subfloat[$128$ points chosen by GILD.\label{fig:plot_ellipse_GILD}]{\includegraphics[width=.25\textwidth]{fig/plot_art2_GILD-crop.pdf}}%
    \hfill\null
    \caption{
    $128$ points (big red circles) of \ellipse selected by greedily maximizing each objective with the Euclidean distance.}
    \label{fig:plot_ellipse}
\end{figure*}%


==> arXiv/fig-recommend.tex <==
\begin{figure*}[ht]
    \centering
    \null\hfill
    \includegraphics[width=.3\textwidth]{fig/recommend_nDCG_nILD.pdf}%
    \hfill%
    \includegraphics[width=.3\textwidth]{fig/recommend_nDCG_ndisp.pdf}%
    \hfill%
    \includegraphics[width=.3\textwidth]{fig/recommend_ndisp_nILD.pdf}%
    \hfill\null
    \caption{
        Relation between each pair of \nDCG, \nILD, and \ndisp with regard to a trade-off parameter $\lambda$.
    }
    \label{fig:recommend}
\end{figure*}


==> arXiv/fig-visualize.tex <==
\begin{figure}[htb]
    \centering
    \subfloat[EILD\label{fig:visualize-hist-ILD_euc}]{\includegraphics[width=.3\textwidth]{fig/visualize/hist_ILD_euc.pdf}}%
    \subfloat[EDISP\label{fig:visualize-hist-disp_euc}]{\includegraphics[width=.3\textwidth]{fig/visualize/hist_disp_euc.pdf}}%
    \subfloat[ILDRBF\label{fig:visualize-hist-ILD_RBF}]{\includegraphics[width=.3\textwidth]{fig/visualize/hist_ILD_RBF.pdf}}%
    \caption{visualize-hist}
    \label{fig:visualize-hist}
\end{figure}


==> arXiv/macro.tex <==
%\usepackage{graphicx}
\usepackage{booktabs,enumitem,multirow}
\usepackage[normalem]{ulem}
\usepackage{framed,fancybox,ascmac}
\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage{diagbox}

\usepackage{nicefrac}
%\usepackage{caption}

\usepackage{mathtools}
\usepackage{apxproof}

\usepackage{comment}
\usepackage{url}
\usepackage[caption=false]{subfig}

%\usepackage[right]{showlabels}
\usepackage{xspace}

\usepackage{bm}

\usepackage[nameinlink]{cleveref}
\usepackage{nameref}

\usepackage{tcolorbox}

\usepackage{lineno}


\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{observation}[theorem]{Observation}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}

\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{claim}{Claim}{Claims}
\crefname{remark}{Remark}{Remarks}
\crefname{observation}{Observation}{Observations}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{appendix}{Appendix}{Appendices}
%\crefformat{section}{#2\S#1#3}
\crefname{section}{Section}{Sections}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{Eq.}{Eqs.}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}

% https://tex.stackexchange.com/questions/561715/how-to-use-a-symbol-as-footnote-marker-with-hyperref-and-cleveref-packages
\crefformat{footnote}{#2\textsuperscript{\normalfont #1}#3}
%\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

\usepackage{algorithmicx}
\usepackage[ruled]{algorithm}
\usepackage[noend]{algpseudocode}
\algnewcommand\And{\; \textbf{and} \;}
\algnewcommand\Or{\; \textbf{or} \;}
\algnewcommand\To{\; \textbf{to} \;}
\algnewcommand\Continue{\textbf{continue}}
\algnewcommand\Not{\textbf{not}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\niceframed}[1]{{\noindent #1}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\median}{median}
\newcommand{\med}{\mathrm{med}}
\renewcommand{\vec}[1]{\mathbf{\bm{#1}}}
\let\det\relax\DeclareMathOperator{\det}{\mathop{\mathrm{det}}}

\renewcommand{\vec}[1]{\mathbf{\bm{#1}}}
\newcommand{\mat}[1]{\mathbf{\bm{#1}}}
\newcommand{\bigO}{\mathcal{O}}

\DeclareMathOperator{\vol}{\mathop{\mathrm{vol}}}
\DeclareMathOperator{\proj}{\mathop{\mathrm{proj}}}
\DeclareMathOperator{\dis}{\mathop{\mathrm{d}}}
\DeclareMathOperator{\sgn}{\mathop{\mathrm{sgn}}}

\newcommand{\ILD}{\textsf{\textup{ILD}}\xspace}
\newcommand{\disp}{\textsf{\textup{disp}}\xspace}
\newcommand{\GILD}{\textsf{\textup{GILD}}\xspace}
\newcommand{\Random}{\textsf{\textup{Random}}\xspace}

\newcommand{\nDCG}{\textsf{\textup{nDCG}}\xspace}
\newcommand{\nILD}{\textsf{\textup{nILD}}\xspace}
\newcommand{\ndisp}{\textsf{\textup{ndisp}}\xspace}

\newcommand{\OPT}{{\mathrm{OPT}}}
\newcommand{\Gr}{{\mathrm{Gr}}}
\DeclareMathOperator{\divf}{\mathop{\mathsf{f}}}
\DeclareMathOperator{\divg}{\mathop{\mathsf{g}}}

\newcommand{\rme}{\mathrm{e}}

\newcommand{\ALG}{\textsc{alg}}

\newcommand{\ML}{\textsl{ML-1M}\xspace}
\newcommand{\Ama}{\textsl{Amazon}\xspace}
\newcommand{\syntha}{\textsl{TwoCircles}\xspace}
\newcommand{\synthb}{\textsl{Ellipse}\xspace}
\newcommand{\circles}{\textsl{TwoCircles}\xspace}
\newcommand{\ellipse}{\textsl{Ellipse}\xspace}
\newcommand{\feedback}{\textsl{feedback}\xspace}
\newcommand{\genre}{\textsl{genre}\xspace}
\newcommand{\easer}{$\textsc{ease}^\textsc{r}$\xspace}

\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}
% calligraphic letters
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

% blackboard bold math capitals
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

% 最終手段
\floatsep=2pt  % 図と図の間のスペース
\dblfloatsep=2pt
%\textfloatsep=6pt  % 本文と図の間のスペース
%\dbltextfloatsep=6pt
\abovecaptionskip=2pt  % 図とキャプションの間のスペース
\belowcaptionskip=2pt  % 図とキャプションの間のスペース
\itemsep=2pt
%\labelsep=0pt
\intextsep=0pt  % 本文中の図のスペース


==> arXiv/tab-relative.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{minipage}[t]{.32\textwidth}
    \renewcommand{\arraystretch}{0.8}
    \center
    \begin{tabular}{c|lll} \toprule
    \multirow{2}{*}{\diagbox{$\divf$}{$\divg$}} & \multicolumn{3}{c}{\textbf{rel.~score} $\divg(S_{\divf,k}^\Gr) / \divg(S_{\divg,k}^\Gr)$} \\
    & \ILD & \disp & \GILD \\ \midrule
    \ILD & -- & 0.424 & 0.997 \\
    \disp & 0.941 & -- & 1.000 \\
    \GILD & \textbf{0.972} & \textbf{0.818} & -- \\
    \Random & 0.345 & 0.053 & 0.934 \\
    \bottomrule
    \end{tabular}
    \caption{Average rel.~score of each pair of diversity objs.~for \feedback on \ML.}
    \label{tab:rel_ml_svd}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.32\textwidth}
    \renewcommand{\arraystretch}{0.8}
    \center
    \begin{tabular}{c|lll} \toprule
    \multirow{2}{*}{\diagbox{$\divf$}{$\divg$}} & \multicolumn{3}{c}{\textbf{rel.~score} $\divg(S_{\divf,k}^\Gr) / \divg(S_{\divg,k}^\Gr)$} \\
    & \ILD & \disp &\GILD \\ \midrule
    \ILD & -- & 0.211 & 0.999 \\
    \disp & 0.975 & -- & 0.998 \\
    \GILD & \textbf{0.997} & \textbf{0.360} & -- \\
    \Random & 0.142 & 0.001 & 0.810 \\
    \bottomrule
    \end{tabular}
    \caption{Average rel.~score of each pair of diversity objs.~for \feedback on \Ama.}
    \label{tab:rel_ama_svd}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.32\textwidth}
    \renewcommand{\arraystretch}{0.8}
    \center
    \begin{tabular}{c|lll} \toprule
    \multirow{2}{*}{\diagbox{$\divf$}{$\divg$}} & \multicolumn{3}{c}{\textbf{rel.~score} $\divg(S_{\divf,k}^\Gr) / \divg(S_{\divg,k}^\Gr)$} \\
    & \ILD & \disp & \GILD \\ \midrule
    \ILD & -- & 0.048 & 0.797 \\
    \disp & 0.859 & -- & 0.936 \\
    \GILD & \textbf{0.889} & \textbf{0.195} & -- \\
    \Random & 0.842 & 0.162 & 0.955 \\
    \bottomrule
    \end{tabular}
    \caption{Average rel.~score of each pair of diversity objs.~for \circles.}
    \label{tab:rel_circles}
    \end{minipage}
    \\
    \begin{minipage}[t]{.32\textwidth}
    \renewcommand{\arraystretch}{0.8}
    \center
    \begin{tabular}{c|lll} \toprule
    \multirow{2}{*}{\diagbox{$\divf$}{$\divg$}} & \multicolumn{3}{c}{\textbf{rel.~score} $\divg(S_{\divf,k}^\Gr) / \divg(S_{\divg,k}^\Gr)$} \\
    & \ILD  & \disp & \GILD \\ \midrule
    \ILD & -- & 0.153 & 0.976 \\
    \disp & 0.959 & -- & 0.999 \\
    \GILD & \textbf{0.970} & \textbf{0.911} & -- \\
    \Random &  0.877 & 0.000 & 0.933 \\
    \bottomrule
    \end{tabular}
    \caption{Average rel.~score of each pair of diversity objs.~for \genre on \ML.}
    \label{tab:rel_ml_genre}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.32\textwidth}
    \renewcommand{\arraystretch}{0.8}
    \center
    \begin{tabular}{c|lll} \toprule
    \multirow{2}{*}{\diagbox{$\divf$}{$\divg$}} & \multicolumn{3}{c}{\textbf{score} $\divg(S_{\divf,k}^\Gr) / \divg(S_{\divg,k}^\Gr)$} \\
    & \ILD & \disp& \GILD \\ \midrule
    \ILD & -- & 0.378 & 0.996 \\
    \disp & 0.979 & -- & 0.999 \\
    \GILD & \textbf{0.989} & \textbf{0.926} & -- \\ 
    \Random & 0.966 & 0.137 & 0.990 \\
    \bottomrule
    \end{tabular}
    \caption{Average rel.~score of each pair of diversity objs.~for \genre  on \Ama.}
    \label{tab:rel_ama_genre}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.32\textwidth}
    \renewcommand{\arraystretch}{0.8}
    \center
    \begin{tabular}{c|lll} \toprule
    \multirow{2}{*}{\diagbox{$\divf$}{$\divg$}} & \multicolumn{3}{c}{\textbf{rel.~score} $\divg(S_{\divf,k}^\Gr) / \divg(S_{\divg,k}^\Gr)$} \\
    & \ILD & \disp& \GILD \\ \midrule
    \ILD & -- & 0.041 & 0.652 \\
    \disp & 0.684 & -- & 1.000 \\
    \GILD & \textbf{0.758} & \textbf{0.272} & -- \\ 
    \Random & 0.567 & 0.185 & 0.985 \\
    \bottomrule
    \end{tabular}
    \caption{Average rel.~score of each pair of diversity objs.~for \ellipse.}
    \label{tab:rel_ellipse}
    \end{minipage}
\end{table*}



==> fig-visualize.tex <==
\begin{figure}[htb]
    \centering
    \subfloat[EILD\label{fig:visualize-hist-ILD_euc}]{\includegraphics[width=.3\textwidth]{fig/visualize/hist_ILD_euc.pdf}}%
    \subfloat[EDISP\label{fig:visualize-hist-disp_euc}]{\includegraphics[width=.3\textwidth]{fig/visualize/hist_disp_euc.pdf}}%
    \subfloat[ILDRBF\label{fig:visualize-hist-ILD_RBF}]{\includegraphics[width=.3\textwidth]{fig/visualize/hist_ILD_RBF.pdf}}%
    \caption{visualize-hist}
    \label{fig:visualize-hist}
\end{figure}

